Thermochemical modelling of brown dwarf discs

The physical properties of brown dwarf discs, in terms of their shapes and sizes, are still largely unexplored by observations. To what extent brown dwarf discs are similar to scaled-down T Tauri discs is currently unknown, and this work is a step towards establishing a relationship through the eventual modelling of future observations. We use observations of the brown dwarf disc $\rho$ Oph 102 to infer a fiducial model around which we build a small grid of brown dwarf disc models, in order to model the CO, HCN, and HCO+ line fluxes and the chemistry which drives their abundances. These are the first brown dwarf models to be published which relate detailed, 2D radiation thermochemical disc models to observational data. We predict that moderately extended ALMA antenna configurations will spatially resolve CO line emission around brown dwarf discs, and that HCN and HCO+ will be detectable in integrated flux, following our conclusion that the flux ratios of these molecules to CO emission are comparable to that of T Tauri discs. These molecules have not yet been observed in sub-mm wavelengths in a brown dwarf disc, yet they are crucial tracers of the warm surface-layer gas and of ionization in the outer parts of the disc. We present the prediction that if the physical and chemical processes in brown dwarf discs are similar to those that occur in T Tauri discs -- as our models suggest -- then the same diagnostics that are used for T Tauri discs can be used for brown dwarf discs (such as HCN and HCO+ lines that have not yet been observed in the sub-mm), and that these lines should be observable with ALMA. Through future observations, either confirmation (or refutation) of these ideas about brown dwarf disc chemistry will have strong implications for our understanding of disc chemistry, structure, and subsequent planet formation in brown dwarf discs.

==> packages.tex <==
\RequirePackage{txfonts}
\RequirePackage{microtype}
\RequirePackage{graphicx}
\RequirePackage{booktabs}
\RequirePackage{amsmath,amssymb}
\RequirePackage{cleveref}
\RequirePackage{pdfpages}
\RequirePackage{textgreek}


\newcommand*{\rangeto}{\textnormal{\hskip.1em\relax--\hskip.1em\relax}}
\RequirePackage[separate-uncertainty=true,range-units=single,range-phrase=\rangeto,forbid-literal-units=true]{siunitx}



% common astronomical symbols
\let\sun\odot
\let\bh\bullet
\newcommand*{\solarmass}{\si{\solarmass}}
\newcommand*{\solarluminosity}{\si{\solarluminosity}}
% astrophysical units
\DeclareSIUnit\lightspeed{$c$}
\DeclareSIUnit\rydberg{Ry}
\DeclareSIUnit\erg{erg}
\DeclareSIUnit\magnitude{mag}
\DeclareSIUnit\jansky{Jy}
\DeclareSIUnit\gauss{G}
\DeclareSIUnit\h{$h$}
\DeclareSIUnit\hseven{$h$_7}
\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\au{AU}
\DeclareSIUnit\year{yr}
\DeclareSIUnit\solarluminosity{\ensuremath{L_\sun}}
\DeclareSIUnit\solarmass{\ensuremath{M_\sun}}
\DeclareSIUnit\jupitermass{\ensuremath{M_\mathrm{J}}}
\DeclareSIUnit\solarmassinenergy{\ensuremath{M_\sun|c^2}}
\DeclareSIUnit\solarradius{\ensuremath{R_\sun}}

% redeclared units
\DeclareSIUnit\arcsecond{as}
%\DeclareSIUnit\astronomicalunit{AU}
\DeclareSIUnit\clight{\ensuremath c}
% additional unit notations
\DeclareRobustCommand\SIfrac{\@ifstar\astrosym@SIfracplain\astrosym@SIfracparen}
%\newcommand*{\astrosym@SIfracplain}[1]{\begingroup\def\@tempa{#1}\astrosym@@SIfracplain}
%\newcommand*{\astrosym@SIfracparen}[1]{\begingroup\def\@tempa{#1}\astrosym@@SIfracparen}
%\newcommand*{\astrosym@@SIfracplain}[2][]{\frac{\@tempa}{\SI{#1}{#2}}\endgroup}
%\newcommand*{\astrosym@@SIfracparen}[2][]{\biggl(\astrosym@@SIfracplain{#1}{#2}\biggr)}
%\newcommand*{\SIex}[2]{#1\,\si{#2}}
% spectroscopic notation
%\DeclareRobustCommand\specatom{\@ifstar\astrosym@atomforbid\astrosym@atomallow}
%\DeclareRobustCommand\specline{\@ifstar\astrosym@lineforbid\astrosym@lineallow}
%\newcommand*{\astrosym@atomforbid}[2]{\textnormal{[\astrosym@atomallow{#1}{#2}]}}
%\newcommand*{\astrosym@atomallow}[2]{%
%  \textnormal{#1\hskip.1em\relax\textsc{\romannumeral#2}}}
%\newcommand*{\astrosym@lineforbid}[3]{%
%  \textnormal{\astrosym@atomforbid{#1}{#2}\hskip.2em\relax#3}}
%\newcommand*{\astrosym@lineallow}[3]{%
%  \textnormal{\astrosym@atomallow{#1}{#2}\hskip.1em\relax#3}}
% term symbol
%\DeclareRobustCommand\termsym{\@ifstar\astrosym@termodd\astrosym@termeven}
%\newcommand*{\scripts}[5]{\ensuremath{
%  ^{#2\vphantom0}_{#3\vphantom0}\hskip-\scriptspace{#1}
%  ^{#4\vphantom0}_{#5\vphantom0}}}
%\newcommand*{\astrosym@termeven}[3]{\scripts{\textup{#2}}{#1}{}{}{#3}}
%\newcommand*{\astrosym@termodd}[3]{\scripts{\textup{#2}}{#1}{}{\textup o}{#3}}
